Visual Embellishments are Potential Distractions in Double-Column Reading

Eye-catching graphics, such as circular figure labels and word-scale visualizations, are increasingly being placed directly within long-form text paragraphs. Some research has claimed that inline visualizations can help readers understand data-rich passages more clearly. However, research in the science of reading calls into question the introduction of images within the flow of text. In this work, we conduct an exploratory study of eye movement in both the presence and absence of visual embellishments. Using a high-resolution eye-tracker (EyeLink Portable Duo), we observed small mean increases in vertical and cross-column saccade rates among six participants, with substantial variation among readers and no detected difference in comprehension accuracy. Mean subjective ratings for the data-light circular-glyph passage indicated it is more distracting than its unembellished comparison passage. These exploratory observations differ from prior findings and motivate a larger, fully crossed study of inline graphics.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> pixel_control_stimuli.tex <==
% \documentclass[11pt]{article}
\usepackage{geometry}
\usepackage{multicol}
\usepackage{lipsum} % For dummy text

% 1. Define the Pixel Ratio (DPI)
% Change 96 to 72 or 300 depending on your target display/output

% 2. Set Page Dimensions
% Replace width and height with your specific pixel values
% Set left, right, top, bottom margins


% 3. Set the Gutter Width (Space between columns)
%\setlength{\columnsep}{606px}
% \setlength{\columnsep}{80px}

% set space between paragraphs
% \usepackage[skip=4pt,indent=0pt]{parskip}

% control vertical spacing between lines
% set stretch is a multiplier of the default
\usepackage{setspace}
% \setstretch{1.0}

% turn off page numbers
\usepackage{nopageno}

%----- FONT SETTINGS ------

% Wallace et al 2022 recommend noto sans and helvetica
% \usepackage[T1]{fontenc}
% \usepackage[utf8]{inputenc}

% Load Noto Sans without making it the document default immediately
\usepackage{noto} 
% Load Helvetica
\usepackage{helvet}
% Load TeX Gyer Terms for Times
\usepackage{newtxtext} 

% Return to standard Serif (if needed)
\newcommand{\useserif}{\fontfamily{ptm}\selectfont}

\newcommand{\usenoto}{\fontfamily{\notosansfamily}\selectfont }

\newcommand{\usehelvet}{\fontfamily{phv}\selectfont}

\newcommand{\usetimes}{\fontfamily{qtm}\selectfont}

%----- END FONT SETTINGS ------

%----- EMBELLISHMENTS  ------
% 
% Here we define a set of name placeholders for shapes
% The \shapeX items are placed in the desired locations
% in the target text (they can repeat).
% Simply add more shape definitions as needed.
% Use a call to renderTemplate to load the text of 
% a document and fill in the relevant shapes and font, e.g.
% \renderTemplate{\blueC}{\blackC}{\blueC}{\usenoto}{energystar.tex}
%
% Packages to make images, from 
% https://www.texready.ir/docs/figures_and_tables/tikz_package
\usepackage{tikz}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{xcolor}
\usetikzlibrary{shadings, arrows.meta}

% define blank shapes to quiet latex errors
\newcommand{\shapeA}{}
\newcommand{\shapeB}{}
\newcommand{\shapeC}{}
\newcommand{\shapeD}{}


% #1=ShapeA, #2=ShapeB, #3=ShapeC, #4=FontMacro, #5=Filename
\newcommand{\renderTemplate}[6]{%
   \clearpage                % Start a fresh page
    #5                        % Apply the font (e.g., \usenoto)
    \renewcommand{\shapeA}{#1\xspace}
    \renewcommand{\shapeB}{#2\xspace}
    \renewcommand{\shapeC}{#3\xspace}
    \renewcommand{\shapeD}{#4\xspace}
    \input{#6}                % Load the specific file provided  
}


\input{shape_definitions}
\input{spark_definitions}
    




==> relatedworkdraft.tex <==
\section{Related Work}
\label{sec:related_work}

\marti{[add something about the split attention model and images far away vs nearby]}

word-scale visualizations
- definition: using text-sized graphics to augment existing documents, from Pascal Goffin, Wesley Willett, Jean-Daniel Fekete, and Petra Isenberg. 2014. Exploring the Placement and Design of Word-Scale Visualizations. IEEE Transactions on Visualization and Computer Graphics 20, 12 (Dec. 2014), 2291–2300.https://doi.org/10.1109/TVCG.2014.2346435
review paper to cite: @inproceedings{lan2026evolving,
  title={The evolving duet of two modalities: a survey on integrating text and visualization for data communication},
  author={Lan, Xingyu and Li, Xi and Zhang, Yixing and Cheng, Mengqin and Wang, Jiazhe and Chen, Siming},
  booktitle={Proceedings of the 2026 CHI Conference on Human Factors in Computing Systems},
  pages={1--19},
  year={2026}
}, also mention Tufte's sparklines (Edward R Tufte. 2001. The visual display of quantitative information. Vol. 2.
Graphics press Cheshire, CT.)
- it has the potential to enhances reading by facilitating users’ understanding of data-rich documents  while  reducing their mental demand and perceived effort (need citation).
For example, when reading code:
 Hoffswell et al. [32] implemented a design space that uses word-scale
visualizations to augment the code reading experience.
(cite Jane Hoffswell, Arvind Satyanarayan, and Jeffrey Heer. 2018. Augmenting Code
with In Situ Visualizations to Aid Program Understanding. In Proceedings of the
2018 CHI Conference on Human Factors in Computing Systems. ACM, Montreal
QC Canada, 1–12. doi:10.1145/3173574.3174106)
For example, 
word-scale visualization can help people understand causality: @article{choudhry2020once,
  title={Once upon a time in visualization: Understanding the use of textual narratives for causality},
  author={Choudhry, Arjun and Sharma, Mandar and Chundury, Pramod and Kapler, Thomas and Gray, Derek WS and Ramakrishnan, Naren and Elmqvist, Niklas},
  journal={IEEE Transactions on Visualization and Computer Graphics},
  volume={27},
  number={2},
  pages={1332--1342},
  year={2020},
  publisher={IEEE}
}

- existing tool has automated the process using language models and visual design knowledge to automatically generate such word-scale visualizations to support such reading facilitation at scale~\cite{zou2025gistvis}, or specific types of word-scale visualizations such as Gestaltlines
(cite @inproceedings{brandes2013gestaltlines,
  title={Gestaltlines},
  author={Brandes, Ulrik and Nick, Bobo and Rockstroh, Brigitte and Steffen, Astrid},
  booktitle={Computer graphics forum},
  volume={32},
  number={3pt2},
  pages={171--180},
  year={2013},
  organization={Wiley Online Library}
})


however, word-scale may not be all good. 
Word-scale visualizations can be of different effectiveness depending on the visualization type, for example, showing Area of interest timeline is better than scan path when expressing eye-tracking data at word-scale (cite: @inproceedings{beck2016expert,
  title={An expert evaluation of word-sized visualizations for analyzing eye movement data},
  author={Beck, Fabian and Acurana, Yasett and Blascheck, Tanja and Netzel, Rudolf and Weiskopf, Daniel},
  booktitle={2016 IEEE Second Workshop on Eye Tracking and Visualization (ETVIS)},
  pages={50--54},
  year={2016},
  organization={IEEE}
})
it can increase reading time, due to the effect of the multiple modalities present in the sentence. (need citation)
For example:
There is evidence that inclusion of images within running text  may have  downstream effects in readability.  In replacing one word in a sentence with a congruent emoji, one study \cite{cohn2018emoji} found that emojis increase reading time but do not have an effect on participant perception of their own comprehension. 
Furthermore, reading time on words following the emoji was also increased relative to no emoji, indicating that the delay in reading does not solely occur when viewing the image. Instead, it may affect the rest of the sentence or further.  
A different  study \cite{barach2021emojis} placed the emoji beside the target word, rather than replacing it.  In this case, participants frequently skipped over the target word when the emoji was included. However, reading time still remained longer for sentences with emoji, as attention was prioritized toward the emoji.
While it is possible that the increased reading time slows people down to support deeper thinking and reflection of the text, it is also possible, from human perception literature, that the existence of the salient visual embellishments distract readers to reduce reading quality.

While the intention of word-scale visualization is not to split viewer attention between figures and text that are not co-located as readers do not have to switch to a separate figure to
read the information \cite{zou2025gistvis}, the existence of these word-scale visualizations, in a way, serve as salient visual embellishment on the text. 
They stand out! And their existence can distract people from reading plain text. 
Work from human perception literature shows that 
(1) salient objects in our peripheral can distract
(2) such distraction can distort things we perceive in the focal points of our vision (
(3) such distraction can reduce higher-level cognition and memory and information-processing. 
But not yet tested in reading and information processing, especially with proefssional scientific journals that requires careful information processing and data intrepretation

Therefore in this work, as a preliminary test, we examine whether the word-scale visualizations in text distract viewers using eye-tracking to see if there are physical disturbances we can observe, and preliminarily examines its effect on reading comprehension and perceived reading experiences. 


\marti{need to update the related work, and be sure to discuss GistVis}



% When text and visuals are spatially separated via a separated figure, to make sense of the content, readers typically exert \textit{voluntary} divided attention, which is a top-down, goal-directed behavior where a reader deliberately coordinates focus between text and figures~\cite{connor2004visual}. 
% Word-scale visualizations that distinctly stand out from the surrounding text, on the other hand, can move readers from a state of voluntary divided attention to \textit{involuntary} divided attention driven by bottom-up attentional capture~\cite{theeuwes2025attentional}. 
% Highly salient, unique visual items automatically trigger attention re-allocation, 
% %within approximately $100\,\mathrm{ms}$, 
% pulling spatial focus away from the primary foveal task regardless of the viewer's intentions \cite{carrasco2011visual, franconeri2003moving}. 



